Diversity-Integration Trade-offs in MIMO Detection

In this work, a MIMO detection problem is considered. At first, we derive the Generalized Likelihood Ratio Test (GLRT) for arbitrary transmitted signals and arbitrary time-correlation of the disturbance. Then, we investigate design criteria for the transmitted waveforms in both power-unlimited and power-limited systems and we study the interplay among the rank of the optimized code matrix, the number of transmit diversity paths and the amount of energy integrated along each path. The results show that increasing the rank of the code matrix allows generating a larger number of diversity paths at the price of reducing the average signal-to-clutter level along each path.

==> abbreviations.tex <==
%%%%% Common LaTeX abbreviations file %%%%%


% Set of real, integer, etc., numbers, l_2 spaces, real, and imaginary parts
\newcommand{\Reals}     {{{\mathrm I\!R}}}  %{{\mathbb R}}
\newcommand{\Cplx}      {{{\mathsf I}\!\!\!{\mathrm C}}} %{{\mathbb C}}
\newcommand{\NCplx}     {{{\mathcal{CN}}}} % Complex normal distribution
\newcommand{\Ints}      {{{\mathbb Z}}} % Z set of all integers
\newcommand{\Rats}      {{{\mathsf I}\!\!\!{\mathrm Q}}}    % Q set of all rational numbers
\newcommand{\Nats}      {{{\mathrm{ I\!N}}}} % N set of all natural numbers
\newcommand{\Tee}{      {{\mathbb T}}}
\newcommand{\ltwo}      {{\ell_2}}
\newcommand{\lone}      {{\ell_1}}
\newcommand{\Ltwo}      {{\mathbb L}^2}
\newcommand{\LtR}       {\Ltwo(\Reals)}
\newcommand{\Real}[1]   {{\mathrm{Re}\left\{#1\right\}}}
\newcommand{\Imag}[1]   {{\mathrm{Im}\left\{#1\right\}}}
\newcommand{\real}      {{\mathcal{R}} e}
\newcommand{\imag}      {{\mathcal{I}} m}

% Some commands for nice typesetting
\newcommand{\ie}        {i.~e., \hspace{2pt}}      % id est
\newcommand{\eg}        {e.~g., \hspace{2pt}}      %
\newcommand{\define}    {\stackrel{\scriptscriptstyle\triangle}{=}}  % define, an '=' with an '^' on top
\newcommand{\D}  {^{\dag}}               % Dagger, includes '^' !
\newcommand{\T}  {{\mathsf{T}}}          % Transpose, no '^' !
\newcommand{\ct} {{\mathsf{*}}}          % conjugate complex, should use \dag for conjugate complex transpose
\newcommand{\half}{{{^1\!\!\scriptscriptstyle{/}\!}_2}}       % a nice 1/2
\newcommand{\mrsss}[1]   {{\mathrm{\scriptscriptstyle{#1}}}}  % math roman scriptscriptstyle - works well for sub and superscripts
\newcommand{\sth}     {{\mathrm{th}}}    % superscript th \th is already defined -- the $k^\sth$ user
\newcommand{\diag}    {{\mathrm{diag}}}  % for diag{1, 2, 3}
\newcommand{\rank}    {{\mathrm{rank}}}  % for diag{1, 2, 3}
\newcommand{\sgn}     {{\mathrm{sgn}}}   % sign function
\newcommand{\tr}      {{\mathrm{tr}}}    % trace of a matrix
\newcommand{\Res}     {{\mathrm{Res}}}   % Residue
\newcommand{\ld}      {{\mathrm{ld}}}    % logarithmus dualis
\newcommand{\barg}    {\overline{\gamma}}     % average received SNR
\newcommand{\sqgb}    {\sqrt{\barg}}     % square root of the average received SNR
\newcommand{\e}       {{\mathrm e}}      % e for exponential function
\newcommand{\E}       {{\mathrm E}}      % Expectation
\newcommand{\lNZ}     {{\lambda_{\mathsf{NZ}}}} % to denote the non-zero eigenvalues of a matrix
\newcommand{\Nt}      {{N_{\!\mrsss{T}}}}% N_T no of transmit antennas
\newcommand{\Nr}      {{N_{\!\mrsss{R}}}}% N_R no of receive antennas
\newcommand{\uple}    {{\mathrm{ul}}}    % upper-left
\newcommand{\upri}    {{\mathrm{ur}}}    % upper-right
\newcommand{\lole}    {{\mathrm{ll}}}    % lower-left
\newcommand{\lori}    {{\mathrm{lr}}}    % lower-right

% Bold numbers
\newcommand{\Zrb}     {{\uwti 0}}      % bold zero
\newcommand{\Oneb}    {{\uwti 1}}      % bold one

% Define bold roman letters
%\newcommand{\uwti}[1]{\mbox{\boldmath $ #1$}}
\newcommand{\uwti}[1]{{\bm #1}}
\newcommand{\ab}{{\uwti a}}  \newcommand{\Ab}{{\uwti A}}
\newcommand{\bb}{{\uwti b}}  \newcommand{\Bb}{{\uwti B}}
\newcommand{\cb}{{\uwti c}}  \newcommand{\Cb}{{\uwti C}}
\newcommand{\db}{{\uwti d}}  \newcommand{\Db}{{\uwti D}}
\newcommand{\eb}{{\uwti e}}  \newcommand{\Eb}{{\uwti E}}
\newcommand{\fb}{{\uwti f}}  \newcommand{\Fb}{{\uwti F}}
\newcommand{\gb}{{\uwti g}}  \newcommand{\Gb}{{\uwti G}}
\newcommand{\hb}{{\uwti h}}  \newcommand{\Hb}{{\uwti H}}
\newcommand{\ib}{{\uwti i}}  \newcommand{\Ib}{{\uwti I}}
\newcommand{\jb}{{\uwti j}}  \newcommand{\Jb}{{\uwti J}}
\newcommand{\kb}{{\uwti k}}  \newcommand{\Kb}{{\uwti K}}
\newcommand{\lb}{{\uwti l}}  \newcommand{\Lb}{{\uwti L}}
\newcommand{\mb}{{\uwti m}}  \newcommand{\Mb}{{\uwti M}}
\newcommand{\nb}{{\uwti n}}  \newcommand{\Nb}{{\uwti N}}
\newcommand{\ob}{{\uwti o}}  \newcommand{\Ob}{{\uwti O}}
\newcommand{\pb}{{\uwti p}}  \newcommand{\Pb}{{\uwti P}}
\newcommand{\qb}{{\uwti q}}  \newcommand{\Qb}{{\uwti Q}}
\newcommand{\rb}{{\uwti r}}  \newcommand{\Rb}{{\uwti R}}
\renewcommand{\sb}{{\uwti s}}\newcommand{\Sb}{{\uwti S}} %\sb is equiv. to _ in Tex, unnecessary.
\newcommand{\tb}{{\uwti t}}  \newcommand{\Tb}{{\uwti T}}
\newcommand{\ub}{{\uwti u}}  \newcommand{\Ub}{{\uwti U}}
\newcommand{\vb}{{\uwti v}}  \newcommand{\Vb}{{\uwti V}}
\newcommand{\wb}{{\uwti w}}  \newcommand{\Wb}{{\uwti W}}
\newcommand{\xb}{{\uwti x}}  \newcommand{\Xb}{{\uwti X}}
\newcommand{\yb}{{\uwti y}}  \newcommand{\Yb}{{\uwti Y}}
\newcommand{\zb}{{\uwti z}}  \newcommand{\Zb}{{\uwti Z}}

% Define bold greek letters, lower and upper case
\newcommand{\alphab}      {{\bm \alpha}}          \newcommand{\Alphab}   {{\uwti {\mathrm A}}}
\newcommand{\betab}       {{\bm \beta}}           \newcommand{\Betab}    {{\uwti {\mathrm B}}}
\newcommand{\gammab}      {{\bm \gamma}}          \newcommand{\Gammab}   {{\bm \Gamma}}
\newcommand{\deltab}      {{\bm \delta}}          \newcommand{\Deltab}   {{\bm \Delta}}
\newcommand{\epsilonb}    {{\bm \epsilon}}        \newcommand{\Epsilonb} {{\uwti {\mathrm E}}}
\newcommand{\varepsilonb} {{\bm \varepsilon}}
\newcommand{\vepsilonb}   {{\bm \varepsilon}}
\newcommand{\zetab}       {{\bm \zeta}}           \newcommand{\Zetab}    {{\uwti {\mathrm Z}}}
\newcommand{\etab}        {{\bm \eta}}            \newcommand{\Etab}     {{\uwti {\mathrm H}}}
\newcommand{\thetab}      {{\bm \theta}}          \newcommand{\Thetab}   {{\bm \Theta}}
\newcommand{\varthetab}   {{\bm \vartheta}}
\newcommand{\vthetab}     {{\bm \vartheta}}
\newcommand{\iotab}       {{\bm \iota}}           \newcommand{\Iotab}    {{\uwti {\mathrm I}}}
\newcommand{\kappab}      {{\bm \kappa}}          \newcommand{\Kappab}   {{\uwti {\mathrm K}}}
\newcommand{\lambdab}     {{\bm \lambda}}         \newcommand{\Lambdab}  {{\bm \Lambda}}
\newcommand{\mub}         {{\bm \mu}}             \newcommand{\Mub}      {{\uwti {\mathrm M}}}
\newcommand{\nub}         {{\bm \nu}}             \newcommand{\Nub}      {{\uwti {\mathrm N}}}
\newcommand{\xib}         {{\bm \xi}}             \newcommand{\Xib}      {{\bm \Xi}}
\newcommand{\omicronb}    {{\uwti {\mathrm o}}} \newcommand{\Omicronb} {{\uwti {\mathrm O}}}
\newcommand{\pib}         {{\bm \pi}}             \newcommand{\Pib}      {{\bm \Pi}}
\newcommand{\varpib}      {{\bm \varpi}}
\newcommand{\vpib}        {{\bm \varpi}}
\newcommand{\rhob}        {{\bm \rho}}            \newcommand{\Rhob}     {{\uwti {\mathrm P}}}
\newcommand{\varrhob}     {{\bm \varrho}}
\newcommand{\vrhob}       {{\bm \varrho}}
\newcommand{\sigmab}      {{\bm \sigma}}          \newcommand{\Sigmab}   {\uwti{\Sigma}}
\newcommand{\varsigmab}   {{\bm \varsigma}}
\newcommand{\vsigmab}     {{\bm \varsigma}}
\newcommand{\taub}        {{\bm \tau}}            \newcommand{\Taub}     {{\uwti {\mathrm T}}}
\newcommand{\upsilonb}    {{\bm \upsilon}}        \newcommand{\Upsilonb} {{\bm \Upsilon}}
\newcommand{\phib}        {{\bm \phi}}            \newcommand{\Phib}     {{\bm \Phi}}
\newcommand{\varphib}     {{\bm \varphi}}
\newcommand{\vphib}       {{\bm \varphi}}
\newcommand{\chib}        {{\bm \chi}}            \newcommand{\Chib}     {{\uwti {\mathrm X}}}
\newcommand{\psib}        {{\bm \psi}}            \newcommand{\Psib}     {{\bm \Psi}}
\newcommand{\omegab}      {{\bm \omega}}          \newcommand{\Omegab}   {{\bm \Omega}}


% Calligraphic letters, normal and bold
\newcommand{\Ac} {{\mathcal A}}         \newcommand{\Ak} {{\bm {\mathcal A}}}
\newcommand{\Bc} {{\mathcal B}}         \newcommand{\Bk} {{\bm {\mathcal B}}}
\newcommand{\Cc} {{\mathcal C}}         \newcommand{\Ck} {{\bm {\mathcal C}}}
\newcommand{\Dc} {{\mathcal D}}         \newcommand{\Dk} {{\bm {\mathcal D}}}
\newcommand{\Ec} {{\mathcal E}}         \newcommand{\Ek} {{\bm {\mathcal E}}}
\newcommand{\Fc} {{\mathcal F}}         \newcommand{\Fk} {{\bm {\mathcal F}}}
\newcommand{\Gc} {{\mathcal G}}         \newcommand{\Gk} {{\bm {\mathcal G}}}
\newcommand{\Hc} {\uwti{\mathcal H}}         \newcommand{\Hk} {{\bm {\mathcal H}}}
\newcommand{\Ic} {{\mathcal I}}         \newcommand{\Ik} {{\bm {\mathcal I}}}
\newcommand{\Jc} {{\mathcal J}}         \newcommand{\Jk} {{\bm {\mathcal J}}}
\newcommand{\Kc} {{\mathcal K}}         \newcommand{\Kk} {{\bm {\mathcal K}}}
\newcommand{\Lc} {{\mathcal L}}         \newcommand{\Lk} {{\bm {\mathcal L}}}
\newcommand{\Mc} {{\mathcal M}}         \newcommand{\Mk} {{\bm {\mathcal M}}}
\newcommand{\Nc} {{\mathcal N}}         \newcommand{\Nk} {{\bm {\mathcal N}}}
\newcommand{\Oc} {{\mathcal O}}         \newcommand{\Ok} {{\bm {\mathcal O}}}
\newcommand{\Pc} {{\mathcal P}}         \newcommand{\Pk} {{\bm {\mathcal P}}}
\newcommand{\Qc} {{\mathcal Q}}         \newcommand{\Qk} {{\bm {\mathcal Q}}}
\newcommand{\Rc} {{\mathcal R}}         \newcommand{\Rk} {{\bm {\mathcal R}}}
\newcommand{\Sc} {{\mathcal S}}         \newcommand{\Sk} {{\bm {\mathcal S}}}
\newcommand{\Tc} {{\mathcal T}}         \newcommand{\Tk} {{\bm {\mathcal T}}}
\newcommand{\Uc} {{\mathcal U}}         \newcommand{\Uk} {{\bm {\mathcal U}}}
\newcommand{\Vc} {{\mathcal V}}         \newcommand{\Vk} {{\bm {\mathcal V}}}
\newcommand{\Wc} {{\mathcal W}}         \newcommand{\Wk} {{\bm {\mathcal W}}}
\newcommand{\Xc} {{\mathcal X}}         \newcommand{\Xk} {{\bm {\mathcal X}}}
\newcommand{\Yc} {{\mathcal Y}}         \newcommand{\Yk} {{\bm {\mathcal Y}}}
\newcommand{\Zc} {{\mathcal Z}}         \newcommand{\Zk} {{\bm {\mathcal Z}}}


\newcommand{\Grb}   {{\uwti {\mathrm V}}}

\newcommand{\Qulk} {{\underline{{\bm {\mathcal Q}}}}}

\newcommand{\Gulc} {{\underline{\mathcal G}}}
\newcommand{\Culc} {{\underline{\mathcal C}}}

% underlined upper and lower case letters
\newcommand{\Aul}  {{\underline A}}              \newcommand{\aul}  {{\underline a}}
\newcommand{\Bul}  {{\underline B}}              \newcommand{\bul}  {{\underline b}}
\newcommand{\Cul}  {{\underline C}}              \newcommand{\cul}  {{\underline c}}
\newcommand{\Dul}  {{\underline D}}              \newcommand{\dul}  {{\underline d}}
\newcommand{\Eul}  {{\underline E}}              \newcommand{\eul}  {{\underline e}}
\newcommand{\Ful}  {{\underline F}}              \newcommand{\ful}  {{\underline f}}
\newcommand{\Gul}  {{\underline G}}              \newcommand{\gul}  {{\underline g}}
\newcommand{\Hul}  {{\underline H}}              \newcommand{\hul}  {{\underline h}}
\newcommand{\Iul}  {{\underline I}}              \newcommand{\iul}  {{\underline i}}
\newcommand{\Jul}  {{\underline J}}              \newcommand{\jul}  {{\underline j}}
\newcommand{\Kul}  {{\underline K}}              \newcommand{\kul}  {{\underline k}}
\newcommand{\Lul}  {{\underline L}}              \newcommand{\lul}  {{\underline l}}
\newcommand{\Mul}  {{\underline M}}              \newcommand{\mull} {{\underline m}}
\newcommand{\Nul}  {{\underline N}}              \newcommand{\nul}  {{\underline n}}
\newcommand{\Oul}  {{\underline 0}}              \newcommand{\oul}  {{\underline o}}
\newcommand{\Pul}  {{\underline P}}              \newcommand{\pul}  {{\underline p}}
\newcommand{\Qul}  {{\underline Q}}              \newcommand{\qul}  {{\underline q}}
\newcommand{\Rul}  {{\underline R}}              \newcommand{\rul}  {{\underline r}}
\newcommand{\Sul}  {{\underline S}}              \newcommand{\sul}  {{\underline s}}
\newcommand{\Tul}  {{\underline T}}              \newcommand{\tul}  {{\underline t}}
\newcommand{\Uul}  {{\underline U}}              \newcommand{\uul}  {{\underline u}}
\newcommand{\Vul}  {{\underline V}}              \newcommand{\vul}  {{\underline v}}
\newcommand{\Wul}  {{\underline W}}              \newcommand{\wul}  {{\underline w}}
\newcommand{\Xul}  {{\underline X}}              \newcommand{\xul}  {{\underline x}}
\newcommand{\Yul}  {{\underline Y}}              \newcommand{\yul}  {{\underline y}}
\newcommand{\Zul}  {{\underline Z}}              \newcommand{\zul}  {{\underline z}}

% Misc. short-cuts
\newcommand{\mc}[1]     {{\mathcal{#1}}}        % mathcal
\newcommand{\what}[1]   {\widehat{#1}}          % widehat
\newcommand{\wtld}[1]   {\widetilde{#1}}        % widetilde
\newcommand{\Portho}[1] {\Pb_{#1}^{\perp}}      % orthogonal projection
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\ds}{\displaystyle}

